Neural Shadow Art

Shadow art is a captivating form of sculptural expression where the projection of a sculpture in a specific direction reveals a desired shape with high precision. In this work, we introduce Neural Shadow Art, which leverages implicit occupancy function representation to significantly expand the possibilities of shadow art. This representation enables the design of high-quality, 3D-printable geometric models with arbitrary topologies at any resolution, surpassing previous voxel- and mesh-based methods. Our method provides a more flexible framework, enabling projections to match input binary images under various light directions and screen orientations, without requiring light sources to be perpendicular to the screens. Furthermore, we allow rigid transformations of the projected geometries relative to the input binary images and simultaneously optimize light directions and screen orientations to ensure that the projections closely resemble the target images, especially when dealing with inputs of complex topologies. In addition, our model promotes surface smoothness and reduces material usage. This is particularly advantageous for efficient industrial production and enhanced artistic effect by generating compelling shadow art that avoids trivial, intersecting cylindrical structures. In summary, we propose a more flexible representation for shadow art, significantly improving projection accuracy while simultaneously meeting industrial requirements and delivering awe-inspiring artistic effects.

==> tables/minipage.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[!t]{0.44\textwidth}

\centering
\caption*{\textbf{Table 2: Comparison of accuracy with the original image.} Our comparison focuses on the alignment between the output projection and the input projection after rigid registration. A higher value indicates that the result is closer to the input image.}
\setlength{\tabcolsep}{2pt} % 调整列之间的间距
% \renewcommand{\arraystretch}{0.9} % 压缩表格的行高
\begin{tabular}{c|cc|cc|cc}
\hline
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{Animal}} & \multicolumn{2}{c|}{\textbf{Currency}} & \multicolumn{2}{c}{\textbf{Music}} \\
 & \textbf{IOU} & \textbf{DS} & \textbf{IOU} & \textbf{DS} & \textbf{IOU} & \textbf{DS} \\
\hline
Shadow Art \cite{MP09} & 0.823 & 0.903 & 0.867 & 0.929 &  0.750 & 0.853 \\
\hline
Shadow Art Revisited & \multirow{2}{*}{0.876} & \multirow{2}{*}{0.934} & \multirow{2}{*}{0.916} & \multirow{2}{*}{0.956} & \multirow{2}{*}{0.901} & \multirow{2}{*}{0.948} \\
 \cite{STR22} (Voxel-based)&  & & & & & \\
\hline
Shadow Art Revisited & \multirow{2}{*}{0.847} & \multirow{2}{*}{0.917} & \multirow{2}{*}{0.870} & \multirow{2}{*}{0.930} & \multirow{2}{*}{0.853} & \multirow{2}{*}{0.920} \\
 \cite{STR22} (Mesh-based)&  & & & & & \\
\hline
Ours & \textbf{0.967} & \textbf{0.983} & \textbf{0.961} & \textbf{0.980} & \textbf{0.952} & \textbf{0.975} \\
\hline
\end{tabular}
\label{tab:accuracy}

    \end{minipage}
    \hfill
    \begin{minipage}[!t]{0.44\textwidth}
\centering
\caption{\textbf{Comparison of surface area and volume of final mesh.} Area and Vol. represent the surface area and volume computed using MeshLab, with the bounding box diameter normalized to 1. The unit of volume is $10^{-2}$.}
\setlength{\tabcolsep}{3pt} % 调整列之间的间距
% \renewcommand{\arraystretch}{0.9} % 压缩表格的行高
\begin{tabular}{c|cc|cc|cc}
\hline
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{Animal}} & \multicolumn{2}{c|}{\textbf{Currency}} & \multicolumn{2}{c}{\textbf{Music}} \\
 & \textbf{Area} & \textbf{Vol.} & \textbf{Area} & \textbf{Vol.} & \textbf{Area} & \textbf{Vol.} \\
\hline
Shadow Art Revisited & \multirow{2}{*}{1.57} & \multirow{2}{*}{4.36} & \multirow{2}{*}{2.02} & \multirow{2}{*}{3.63} & \multirow{2}{*}{1.05} & \multirow{2}{*}{2.61} \\
 \cite{STR22} (Voxel-based)&  & & & & & \\
\hline
Ours & \textbf{1.03} & \textbf{3.35} & \textbf{1.04} & \textbf{2.13} & \textbf{0.76} & \textbf{1.93} \\
\hline
\end{tabular}
\label{tab:volume}



    \end{minipage}
\end{figure*}
